Do different prompting methods yield a common task representation in language models?

Demonstrations and instructions are two primary approaches for prompting language models to perform in-context learning (ICL) tasks. Do identical tasks elicited in different ways result in similar representations of the task? An improved understanding of task representation mechanisms would offer interpretability insights and may aid in steering models. We study this through \textit{function vectors} (FVs), recently proposed as a mechanism to extract few-shot ICL task representations. We generalize FVs to alternative task presentations, focusing on short textual instruction prompts, and successfully extract instruction function vectors that promote zero-shot task accuracy. We find evidence that demonstration- and instruction-based function vectors leverage different model components, and offer several controls to dissociate their contributions to task performance. Our results suggest that different task promptings forms do not induce a common task representation through FVs but elicit different, partly overlapping mechanisms. Our findings offer principled support to the practice of combining instructions and task demonstrations, imply challenges in universally monitoring task inference across presentation forms, and encourage further examinations of LLM task inference mechanisms.

==> tables/localizer_results_table.tex <==
\begin{table}[!tp]
\centering
\resizebox{\textwidth}{!}{%
% \begin{adjustbox}{center}
\begin{threeparttable}
\caption{\textbf{Localization experiments demonstrate asymmetry between demonstrations and instructions.}  }
\label{tab:localizer-results}


% \begin{tabular}{p{3.5cm}p{\LocalizerColWidth}p{\LocalizerColWidth}p{\LocalizerColWidth}p{\LocalizerColWidth}}

\begin{tabular}{lllllllr}
\toprule
\textbf{Evaluation} & \textbf{Intervention} & \textbf{Llama-3.2-3B}     & \textbf{3.2-3B-Instruct}   & \textbf{Llama-3.1-8B}     & \textbf{3.1-8B-Instruct}   &   \textbf{Mean $\Delta$} \\
\midrule
 \multirow{3}{3em}{Shuffled 10-shot} & Demonstration FV             & 0.7083           & 0.7907                  & 0.5142           & 0.7372                  &                   \\
 & \makecell[cl]{ Instruction heads \& \\ Demonstration acts } & 0.0936 (-0.6147) & 0.4170 (-0.3737)        & 0.1100 (-0.4043) & 0.3534 (-0.3838)        &           -0.4441 \\
& \makecell[cl]{ Demonstration heads \& \\ Instruction acts }   & 0.2146 (-0.4937) & 0.2556 (-0.5350)        & 0.1842 (-0.3301) & 0.2283 (-0.5089)        &           -0.4669 \\
 \midrule
 \multirow{3}{*}{0-shot} & Instruction FV                    & 0.4550           & 0.5546                  & 0.2321           & 0.5753                  &                   \\
 & \makecell[cl]{ Instruction heads \& \\ Demonstration acts } & 0.3003 (-0.1547) & 0.4148 (-0.1397)        & 0.1602 (-0.0719) & 0.4613 (-0.1140)        &           -0.1201 \\
 & \makecell[cl]{ Demonstration heads \& \\ Instruction acts } & 0.2152 (-0.2398) & 0.1969 (-0.3576)        & 0.2032 (-0.0289) & 0.1870 (-0.3883)        &           -0.2537 \\
\bottomrule
\end{tabular}
% \begin{tablenotes}
%     \item We observe consistently higher causal indirect scores for instruction FV heads in the demonstration setting, compared to using demonstration FV heads in the instruction setting (``localizer difference,'' highlighted).

%     \item This effect is not merely due causal effects being higher in the demonstration setting; the first and last row provide the median CIE in each condition, and we observe that the median CIE in the instruction setting is higher in every case, by as much as an order of magnitude for some models. 
    
% \end{tablenotes}
\end{threeparttable}
}
% \end{adjustbox}
\end{table}

==> tables/method_diffs_summary_table.tex <==
\begin{table}[!bthp]
\centering
% \begin{adjustbox}{center}
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\caption{\textbf{Summary of method differences}}
\label{tab:rqs}
% \begin{tabular}{|p{3cm}|rrl|rrl|rrl|}

\begin{tabular}{p{2.25cm}p{6cm}p{6cm}}

\toprule

 & \textbf{Demonstrations} \citep{Todd2024-xr} & \textbf{Instructions} (ours) \\
\midrule
\textbf{Dataset} $D_t$ & \multicolumn{2}{c}{\small $\{ (x_1 = \text{Japan}, y_1 = \text{Tokyo}), (x_2 = \text{Chile}, y_2 = \text{Santiago}), (x_3 = \text{France}, y_3 = \text{Paris}), \cdots \}$  } \\
\textbf{Query} $(x_{iq}, y_{iq})$ & \multicolumn{2}{c}{\small $(x_{iq} = \text{Egypt}, y_{iq} = \text{Cairo})$ } \\
\textbf{Prompt} $p_i^t$ & \makecell[cl]{Q: Japan. A: Tokyo.\\ Q: Chile. A: Santiago. \\ ... \\ Q: France. A: Paris. \\ Q:  Egypt. A:  } & \makecell[tl]{Map from a country to its capital. \\ Q: Egypt. A: } \\
\textbf{Uninformative prompt} $\tilde{p}_i^t$ & \makecell[cl]{Q: Japan. A: Paris.\\ Q: Chile. A: Tokyo. \\ ... \\ Q: France. A: Santiago. \\ Q:  Egypt. A:  } & \makecell[tl]{\textbf{Equiprobable: TODO: sample here}. \\ Q: Egypt. A: \\ \textbf{Real text: TODO: sample here} \\ \textbf{Other task propmt: sample here} } \\

\bottomrule
\end{tabular}
% \begin{tablenotes}
%     \item \textbf{Do we need any notes?}
% \end{tablenotes}
\end{threeparttable}
}
% \end{adjustbox}
\end{table}
